A Database of Modular Forms on Noncongruence Subgroups

We present a database of several hundred modular forms up to and including weight six on noncongruence subgroups of index $\leq 17$. In addition, our database contains expressions for the Belyi map for genus zero subgroups and equations of the corresponding elliptic curves for genus one subgroups and numerical approximations of noncongruence Eisenstein series to 1500 digits precision.

==> subgroups.tex <==
\section{Exhaustive generation of finite index subgroups of $\mathrm{PSL}_2(\ZZ)$}
\label{sec:subgroups_computation}
In this section we outline an algorithm for generating all conjugacy classes of index $\mu$ subgroups in $\mathrm{PSL}_2(\ZZ)$. The current version of the database only includes data for $\mu\le 17$, so we may simply use the database~\cite{stroemberg_db} made by Str\"omberg. However, to extend the database further one would need to list conjugacy classes of subgroups of index $18$ and higher, and the algorithm for listing subgroup classes used by Str\"omberg and described in~\cite[Sec.~7.1]{stroemberg_recent} gets prohibitively expensive to run for larger values of $\mu$.

As is well known {\color{red}(and explained in Section~?? above)}, the problem of generating conjugacy class representatives for all subgroups of index $\mu$ in $\mathrm{PSL}_2(\ZZ)$ is equivalent to that of generating all pairs $(\sigma_S, \sigma_R)$ of permutations in $S_{\mu}$, up to conjugation, such that $\sigma_S^2=\sigma_R^3=1$ and the group generated by $\sigma_R$ and $\sigma_S$ is transitive. This problem can be split into two parts: (1) find a way to generate a list of pairs $(\sigma_S, \sigma_R)$ that contains all possible conjugacy classes of admissible pairs and (2) for each pair $(\sigma_S, \sigma_R)$ from find some canonical representative modulo conjugation in $S_{\mu}$. Provided that the procedure in part (2) is sufficiently efficient, the main goal is then to make the generation procedure in part (1) to not produce equivalent pairs very often. 

Part (2) can be achieved using the SmallestImageSet function (implemented by Steve Linton) from the GRAPE package for GAP {\color{red}(give proper citation)}. To get a canonical representative of the pair $(\sigma_S, \sigma_R)$ we first apply conjugation to put $\sigma_R$ into a canonical form $(1\,2\,3)(4\,5\,6)\dots$ (i.e. we list $k$ 3-cycles in order and then make the points $n-l+1,\dots,n$ to be fixed, where the cycle type of $\sigma_R$ is $3^l1^k$ with $n=3k+l$) and then find the lexicographically smallest representative for $\sigma_S$ under the action of the centralizer of $\sigma_R$ (we view $\sigma_S$ as a set of transpositions, and to quickly find a lexicographically minimal set in an orbit under the action of a permutation group we use the above mentioned SmallestImageSet function).

For part (1), we need the following construction. To each pair $(\sigma_S, \sigma_R)$ with $\sigma_R$ of cycle type $1^l3^k$ with $n=3k+l$ we assign a connected graph $\Sigma$, whose vertices are the orbits of $\sigma_R$, ane edges are the transpositions of $\sigma_S$, with an edge $(i\,j)$ connecting the orbit of $i$ with the orbit of $j$. Under this assignment $\Sigma$ is a graph, possibly with loops and double or even triple edges, whose vertices we color in black or white, according to whether the orbit is of size $3$ or $1$. Then the vertex degree of any black vertex is $\le 3$, and the vertex degree of any white vertex is $\le1$, conjugate pairs of permutations give rise to isomorphic graphs, and the graph $\Sigma$ is connected if and only if the group $\langle\sigma_S,\sigma_R\rangle$ is transitive. 

To generate all (conjugacy class representatives of) pairs $(\sigma_S, \sigma_R)$ we fix some canonical choice of $\sigma_R$ and generate isomorphism classes of connected graphs $\Sigma$ with vertices of two types and above degree restrictions. Isomorph-free generation of $\Sigma$'s can be done efficiently by adapting Brendan McKay's program \textsc{nauty} {\color{red}(add citation)}. Then for  fixed $\sigma_R$ and $\Sigma$ we generate $\sigma_S$ in all possible ways by choosing the transpositions connecting appropriate orbits corresponding to each edge of $\Sigma$; this can be done by a simple recursive procedure. A final optimization is to note that the subgroup of the centralizer of $\sigma_R$ that preserves the partition into orbits leaves $\Sigma$ (and $\sigma_R$) invariant, and hence can be used to modify $\sigma_S$ without changing the conjugacy class. To deal with this extra freedom we pick any maximal matching in $\Sigma$ (including all loops, if any), and assign the corresponding transpositions in $\sigma_S$ in an arbitrary but fixed way (respecting the graph $\Sigma$, of course). It is not hard to see that with this procedure any any conjugacy class of pair $(\sigma_S,\sigma_R)$ will appear at most $|\mathrm{Aut}\Sigma|\cdot 3^{k'}$ times, where $k'$ is the number of black vertices that are not in the chosen maximal matching of $\Sigma$.

We have implementated the above algorithm in \textsc{Sage}, and with this implementation one can generate all conjugacy classes of subgroups of $\mathrm{PSL}_2(\ZZ)$ of index $24$ in just a few hours.
